Lyapunov criteria for robust forward completeness of distributed parameter systems

We show that the robust forward completeness for distributed parameter systems is equivalent to the existence of a corresponding Lyapunov function that increases at most exponentially along the trajectories.

==> Abkuerzungen.tex <==
	
%
%\newtheorem{Satz}{Satz}[section]    %for model ~(\ref{OekosystemModell}
%\newtheorem{Hyp}{Hypothese}[section]  %for model ~(\ref{OekosystemModell}
%
%\newtheorem{Lemm}{Lemma}[section]    %for model ~(\ref{OekosystemModell}
%\newtheorem{Def}{Definition}[section]  
%\newtheorem{remark}[Lemm]{Bemerkung}
%
%\newtheorem  {corollary}[Satz]   {Korollar}
%%\newtheorem* {corollary*}           {Corollary}
%\newtheorem  {proposition}[Satz] {Proposition}
%
%\newtheorem  {examp}[Satz]     {Beispiel}
%%\newtheorem* {examp*}          {Example}
%\newtheorem  {exps}[Satz]      {Beispiele}
%
%\newtheorem{Ass}{Voraussetzung}[section]  
%
%
%\newtheorem{Ex}{Aufgabe}[section] 
%\newtheorem{Sol}{Lösung}[section] 
%%\newtheorem*{Sol*}{Solution}[section] 
%\newtheorem*{Sol*}{Lösung} 





\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{hyp}{Conjecture}[section]  %for model ~(\ref{OekosystemModell}
%
%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
%%\newtheorem{xca}[theorem]{Exercise}
%

\newtheorem{ass}{Assumption}[section]  
\newtheorem{exercise}{Exercise}[section] 
\newtheorem{solution}{Solution}[section] 
\newtheorem*{solution*}{Solution} 
\newtheorem{openprob}[theorem]{Open Problem}


%\newtheorem{nnremark}[theorem]{\sc Remark}
\newtheorem{nnremark}[theorem]{\bf Remark}
\newenvironment{remark}{\begin{nnremark} \rm }{\hfill \hspace*{1pt}\hfill $\lrcorner$\end{nnremark}}

%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
%

%\newtheorem{Satz}{Theorem}[section]    %for model ~(\ref{OekosystemModell}


%\newtheorem{Lemm}{Lemma}[section]    %for model ~(\ref{OekosystemModell}
%\newtheorem{Def}{Definition}[section]  
%\newtheorem{remark}[Lemm]{Remark}

%\newtheorem  {corollary}[Satz]   {Corollary}
%\newtheorem* {corollary*}           {Corollary}
%\newtheorem  {proposition}[Satz] {Proposition}

%\newtheorem  {examp}[Satz]     {Example}
%\newtheorem* {examp*}          {Example}
%\newtheorem  {exps}[Satz]      {Examples}

%
%%%%%%%%%%%%%%%%%%%%%%%%%   Start: From Halbgruppentheorie Skript %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
%
%
%
%% Das Differential-d, aus der Klasse bgteubner
%\makeatletter
%\let\origd=\d
%\renewcommand*\d{
  %\relax\ifmmode
    %\mathrm{d}%
  %\else
    %\expandafter\origd
  %\fi
%}\makeatother
%
%\newcommand \BetragFett  {\mbox{\rule[-1 mm]{0.75 mm}{4.5 mm}}}
%
%\newcommand \items {\item \underline{Schritt:}~}
%
%
%
%
%
%\newcommand{\Kb}{\mathbb{K}}
%\newcommand{\Kntn}{\Kb^{n \times n}}
%%\newcommand{\N}{\mathbb{N}}
%%\newcommand{\K}{\ensuremath{\mathcal{K}}}
%%\newcommand{\Linf}{L_{\infty}}
%
%\newcommand{\supp}{\text{supp}}
%\newcommand{\rank}{\text{rank}}
%
%
%
%\newcommand{\pder}[2][]{\frac{\partial#1}{\partial#2}}
%\newcommand{\scalp}[2]{ \lel #1, #2 \rir }
%
%
%\makeatletter % changes the catcode of @ to 11
%\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
%\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
%\makeatother % changes the catcode of @ back to 12
%
%\newcounter{syscounter}
%\newenvironment{sysnum}{\begin{list}{($\Sigma{\arabic{syscounter}}$)}%
%{\settowidth{\labelwidth}{($\Sigma4$)}
%\settowidth{\leftmargin}{($\Sigma4$)~}%
%\usecounter{syscounter}}}
%{\end{list}}
%
%%
%%\newcounter{syscounter}
%%\newenvironment{sysnum}{\begin{list}{($\Sigma{\arabic{syscounter}}$)}%
%%{\settowidth{\labelwidth}{($\Sigma4$)}
%%\settowidth{\leftmargin}{($\Sigma4$)~}%
%%\usecounter{syscounter}}}
%%{\end{list}}
%%
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%   End: From Halbgruppentheorie Skript %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
%
%
%
%%\numberwithin{equation}{chapter}
%%
%%\newtheoremstyle{thm}%      name
  %%{\baselineskip}%          Space above
  %%{\baselineskip}%          Space below
  %%{\upshape}%               Body font
  %%{}%                       Indent amount (empty = no indent, \parindent = para indent)
  %%{\bfseries}%              Thm head font
  %%{\\}%                       Punctuation after thm head
  %%{.5em}%                   Space after thm head: " " = normal interword space;
        %%%                   \newline = linebreak
  %%{}%                       Thm head spec (can be left empty, meaning `normal')
%%
%%\newtheoremstyle{others}%   name
  %%{\baselineskip}%          Space above
  %%{\baselineskip}%          Space below
  %%{\upshape}%               Body font
  %%{}%                       Indent amount (empty = no indent, \parindent = para indent)
  %%{\bfseries}%              Thm head font
  %%{\\}%                       Punctuation after thm head
  %%{.5em}%                   Space after thm head: " " = normal interword space;
        %%%                   \newline = linebreak
  %%{}%                       Thm head spec (can be left empty, meaning `normal')
%%
%%\newtheoremstyle{TableFigure}%   name
  %%{\baselineskip}%          Space above
  %%{\baselineskip}%          Space below
  %%{\upshape}%               Body font
  %%{}%                       Indent amount (empty = no indent, \parindent = para indent)
  %%{\bfseries}%              Thm head font
  %%{}%                       Punctuation after thm head
  %%{.5em}%                   Space after thm head: " " = normal interword space;
        %%%                   \newline = linebreak
  %%{}%                       Thm head spec (can be left empty, meaning `normal')
%
%
%%\theoremstyle{thm}
%%\newtheorem  {theorem}{Theorem}
%%
%%\newtheorem  {satz}        {Satz}[chapter]
%%\newtheorem* {satz*}                {Satz}
%%\newtheorem  {defsatz}[satz]     {Definition und Satz}
%%\newtheorem  {corollary}[satz]   {Corollary}
%%\newtheorem* {corollary*}           {Corollary}
%%\newtheorem  {proposition}[satz] {Proposition}
%%\newtheorem  {lemma}[satz]       {Lemma}
%%
%%\theoremstyle{others}
%%\newtheorem* {property}      {Property}
%%\newtheorem  {remark}[satz]      {Remark}
%%\newtheorem* {remark*}              {Remark}
%%\newtheorem  {test}[satz] {Test}
%%\newtheorem  {definition}[satz]  {Definition}
%%\newtheorem* {definition*}          {Definition}
%%\newtheorem  {defrem}[satz]      {Definition and remark}
%%\newtheorem* {reminder}             {Erinnerung}
%%\newtheorem  {examp}[satz]     {Example}
%%\newtheorem* {examp*}             {Example}
%%\newtheorem  {exps}[satz]           {Examples}
%%\newtheorem  {notation}[satz]    {Notation}
%%\newtheorem* {notation*}            {Notation}
%%\newtheorem  {claim}[satz]       {Claim}
%%\newtheorem*  {claim*}              {Claim}
%%\newtheorem  {assumption}  {Assumption}
%%\newtheorem*  {assumption*}              {Assumption}
%%\newtheorem*  {comment*}              {Comment}
%%
%%\theoremstyle{TableFigure}
%%\newtheorem {newtable}[equation]        {Tabelle}
%%\newtheorem {newfigure}[equation]       {Abbildung}
%%
%%\newenvironment{alphenumi}%
%%    {\renewcommand{\labelenumi}{\alph{enumi})}\begin{enumerate}}
%%    {\end{enumerate}}
%%\newenvironment{adenumi}%
%%    {\renewcommand{\labelenumi}{{ad} \arabic{enumi})}\begin{enumerate}}
%%    {\end{enumerate}}
%%\newenvironment{adalphenumi}%
%%    {\renewcommand{\labelenumi}{ad (\alph{enumi})}\begin{enumerate}}
%%    {\end{enumerate}}
%%\newenvironment{undlinenumi}
%%        {\renewcommand{\labelenumi}{\underline{\arabic{enumi}.}}\begin{enumerate}}
%%        {\end{enumerate}}

